From Gradient Flow on Population Loss to Learning with Stochastic Gradient Descent

Stochastic Gradient Descent (SGD) has been the method of choice for learning large-scale non-convex models. While a general analysis of when SGD works has been elusive, there has been a lot of recent progress in understanding the convergence of Gradient Flow (GF) on the population loss, partly due to the simplicity that a continuous-time analysis buys us. An overarching theme of our paper is providing general conditions under which SGD converges, assuming that GF on the population loss converges. Our main tool to establish this connection is a general converse Lyapunov like theorem, which implies the existence of a Lyapunov potential under mild assumptions on the rates of convergence of GF. In fact, using these potentials, we show a one-to-one correspondence between rates of convergence of GF and geometrical properties of the underlying objective. When these potentials further satisfy certain self-bounding properties, we show that they can be used to provide a convergence guarantee for Gradient Descent (GD) and SGD (even when the paths of GF and GD/SGD are quite far apart). It turns out that these self-bounding assumptions are in a sense also necessary for GD/SGD to work. Using our framework, we provide a unified analysis for GD/SGD not only for classical settings like convex losses, or objectives that satisfy PL / KL properties, but also for more complex problems including Phase Retrieval and Matrix sq-root, and extending the results in the recent work of Chatterjee 2022.

==> files/appx_application_matrix_sqrt_old.tex <==
\subsection{Matrix square root} 
\begin{lemma}[Self-bounding of \(F\)] \ascomment{Clean!}
\label{lem:f_sb_matrix_sqrt} 
For any matrix \(W\), 
\begin{align*}
 \nrm*{\grad F(W)}_F^2 &\leq 4 F(W)^{3/2} + 4 \smax(M) F(W). 
 \end{align*}
\end{lemma} 
\begin{proof} Since \(\grad F(w) = (W^2 - M) W  +  W (W^2 - M)\), we have  
\begin{align*}
\nrm{\grad F(W)}^2_F &\leq 2 \nrm{(W^2 - M) W }^2_F + 2 \nrm{W (W^2 - M)}^2_F \\
&\leq 4 \smax(W)^2 \nrm{W^2 - M}^2_F \\
&\leq 4 \smax(W^2) F(W), 
\end{align*}
where the last line holds because \(W\) is PD and thus \(\smax(W)^2 = \smax(W^2)\), and by using the definition of \(F(W)\). Using the fact that 
\begin{align*}
 \smax(W^2) &\leq  \smax(W^2 - M) + \smax(M)  \leq \nrm{W^2 - M}_F + \smax(M) = \sqrt{F(W)} + \smax(M)
\end{align*}
in the above, we get  
\begin{align*}
 \nrm*{\grad F(w)}_F^2 &\leq 4 F(W)^{3/2} + 4 \smax(M) F(W). 
 \end{align*}
\end{proof}



\subsubsection{Rate of convergence for gradient flow} 
\begin{lemma}[Modification of Lemma 4.2 in \cite{jain2017global}] 
\label{lem:matrix_sqrt_gfprop1} 
Suppose W(t) is the point obtained by running gradient flow for \(t\) time starting from the point \(W\). If W is PD, then $W(t)$ is also PD, and has minimum singular value bounded by: 
\begin{align*}
\smin(W(t)) &\geq \min \crl*{ \smin(W), \sqrt{\frac{\smin(M)}{10}}}. 
\end{align*} 
\end{lemma} 
\begin{proof} \ascomment{Add proof here that $W(t)$ is also PD; The following proof is incomplete right now. The proof is indentical to the proof of Lemma 4.2 in Jain et. al.} 

We now proof the desired lower bounds on \(\smin(W(t))\). Fix any \(t > 0\). In order to prove the result for the point \(W(t)\), we discretize the time interval \([0, t]\) into \(K_\delta = \ceil*{\frac{t}{\delta}}\) many intervals whose end points are given by \(\crl{0, \delta, 2 \delta, \dots, t - \delta, t}\), where \(\delta > 0\)  and will be fixed later. Furthermore, for any \(k \leq K_\delta\), we define the point \(\bW(k)\) using the recursive relation
\begin{align*}
\bW(k) = \begin{cases}
W & \text{if $k = 0$} \\
\bW(k - 1) - \delta \grad F(\bW(k-1)) & \text{if $k \geq 1$}. 
\end{cases}.  \numberthis \label{eq:msq_PL_1} 
\end{align*}

Since the function \(F\) is \(\bbC_\infty\), we have that \(\lim_{\delta \rightarrow 0} \bW(K_{\delta}) = W(t)\). In the following, we will show via induction that for any \(k \leq K\), the point \(\bW(k)\) satisfies the bound 
\begin{align*}
\ascomment{fill}   \numberthis \label{eq:msq_PL_2}  
\end{align*}

The base case for \(k = 0\) follows trivially. In order to prove the induction step, suppose \pref{eq:msq_PL_2} holds for any \(k' \leq  k\), in the following we will show that \pref{eq:msq_PL_2} also holds for \(k + 1\). First note that 
\begin{align*}
\smin(\bW(k + 1)) &=  \smin\prn*{\bW_k - \delta(\bW_k - M) \bW_k  - \delta  \bW_k (\bW_k - M)}  && \text{(using \pref{eq:msq_PL_1})} \\ 
&= \ascomment{fill} 
\end{align*}
	
\end{proof} 


\begin{lemma}[Lemma 4.5 in \cite{jain2017global}] 
\label{lem:matrix_sqrt_gfprop2} 
For any point \(W\), the function \(F(W) = \nrm*{W^2 - M}^2\) satisfies 
\begin{align*}
\nrm*{\grad F(W)}_F^2 \geq 4 \smin^2(W) F(W). 
\end{align*} 
\end{lemma}

The above two properties give us the following convergence guarantee for gradient flow when starting from any PD point \(W\). 

\begin{lemma} 
\label{lem:PD_matrix_sqrt_gf_convergence} 
Let the starting point \(W\) be PD, let the point \(W(t)\) obtained by running gradient flow for \(t\) time when starting from the point \(W\) satisfies 
\begin{align*}
F(W(t)) \leq F(W(0)) \exp\prn*{- 4 t \min \crl*{ \smin(W), \sqrt{\frac{\smin(M)}{10}}}}. 
\end{align*}
\end{lemma}
\begin{proof} Using chain rule, we get
\begin{align*}
\frac{\dif F(W(t))}{\dif (t)} &= \tri*{\grad F(W(t)), \dot{W}(t)} \\
&= - \nrm*{\grad F(W(t))}_F^2  && \text{(since \( \dot{W}(t) = - \grad F(W(t))\))} \\
&\leq - 4 \smin^2(W(t)) F(W(t))  && \text{(using \pref{lem:matrix_sqrt_gfprop2})} \\ 
&\leq - 4 \min \crl*{ \smin(W)^2, \frac{\smin(M)}{10}} F(W(t)) && \text{(using \pref{lem:matrix_sqrt_gfprop1})} 
\end{align*}
	
Noting that \(F(W(t)) > 0\), rearranging both the sides and integrating with respect to \(t\), we get that 
\begin{align*}
\int_{\tau = 0}^t \frac{1}{F(w(\tau))} \dif F(W(t)) &\leq - 4 \min \crl*{ \smin(W)^2, \frac{\smin(M)}{10}}  \int_{\tau = 0}^t \dif t. 
\end{align*}

The above implies that 
\begin{align*}
F(W(t)) \leq F(W(0)) \exp\prn*{- 4 t \min \crl*{ \smin(W)^2, \frac{\smin(M)}{10}} }, 
\end{align*}
the desired statement follows by noting that \(W(0) = W\). 
\end{proof}

\begin{lemma} 
\label{lem:matrix_sqrt_gf_convergence_nonsmooth} 
 Let point \(W(t)\) obtained by running gradient flow for \(t\) time when starting from the point \(W\) satisfies 
\begin{align*} 
F(W(t)) \leq F(W(0)) \exp\prn*{- 4 t \min \crl*{ \smin(W)^2, \frac{\smin(M)}{10}} }. 
\end{align*}
\end{lemma}

Since the rate in the above Lemma is not smooth in \(W\), we can relax it by using the following softmin approximation to \(\smin(W)\). 

\begin{definition} For any \(\lambda > 0\), define the function\footnote{Whenever clear from the context, we will drop the subscript \(\lambda\) from the function \(h_\lambda\) to simplify the notation.}  
\begin{align*}
h_\lambda(W) = - \frac{1}{\lambda} \log \prn*{\trace{\exp(- \lambda W)} + \exp\prn*{- \frac{\lambda \smin(M)}{10}}}.  
\numberthis \label{eq:matrix_sqrt_h_defn} 
\end{align*}
\end{definition}

The following lemma relates \(h_\lambda(W)\) and \(\smin(W)\). 
\begin{lemma}  
\label{lem:matrix_softmin_properties} 
For any \(W\), 
 \begin{align*}
h_\lambda(W^2) \leq \min \crl*{ \smin(W)^2, \frac{\smin(M)}{10}} \leq h_\lambda(W^2) + \frac{\log(d + 1)}{\lambda}. 
\end{align*}
\end{lemma}
\ascomment{Note that we made an implicit assumption that \(W\) is symmetric.} 
\begin{proof}
	\ascomment{Complete the proof here. The proof in the following is for the scalar case!} 
	
-------------- 
Since \(\log(\cdot)\) is a monotonic function, we have that 
\begin{align*} 
h_\lambda(w) &= - \frac{1}{\lambda} \log \prn*{\sum_{k=1}^d e^{- \lambda w[k]}} \leq -\frac{1}{\lambda} \log \prn*{e^{-\lambda \min_k \prn{w[k]}}} = \min_k \prn{w[k]}.
\end{align*}

We also have that: 
\begin{align*}
h_\lambda(w) &= - \frac{1}{\lambda} \log \prn*{\sum_{k=1}^d e^{- \lambda w[k]}} \geq  -\frac{1}{\lambda} \log \prn*{d e^{-\lambda \min_k \prn{w[k]}}}   \geq  \min_k \prn{w[k]} - \frac{\log(d)}{\lambda}. 
\end{align*}
--------------- 
\end{proof}

Using the relation in \pref{lem:matrix_softmin_properties}  in \pref{lem:matrix_sqrt_gf_convergence_nonsmooth}  suggests that the following rate guarantee also holds. 
\begin{corollary}
\label{corr:matrix_sqrt_gf_convergence}  
Let \(\lambda > 0\). Let \(W(t)\) be the point obtained by running gradient flow for \(t\) time when starting from the point \(W\), then \(W(t)\) satisfies 
\begin{align*} 
F(W(t)) \leq F(W(0)) \exp\prn*{- 4 t \cdot h_\lambda(W^2(0))}. 
\end{align*} 
\end{corollary}

\subsubsection{Potential function} 
\begin{lemma} The potential function \(\Phi\) defined as: 
\begin{align*}
\Phi(W) = \frac{F(W)}{4 h_\lambda(W)}  \numberthis  \label{eq:matrix_sqrt_potential_def}  
\end{align*}
satisfies \pref{def:admissible_potential_self-bounding} for the function \(F\) and the rate given in \pref{corr:matrix_sqrt_gf_convergence}. 
\end{lemma}  
\begin{proof} We define the following generalized potential: 
\begin{align*} 
\Phi(W) &= \int_{t=0}^\infty R(W, t) \dif t =  \int_{t=0}^\infty F(W(0)) \exp\prn*{- 4 t \cdot h_\lambda(W(0))} \dif t = \frac{F(W)}{4h_\lambda(W)}. 
\end{align*} 
\end{proof}

%We now show the self-bounding property of the potential: 
%\begin{lemma}
%	
%\end{lemma}
%\begin{proof} First note that: 
%\begin{align*}
%\grad \Phi(w) &= 4 \frac{w^3 - m w}{h(w)^2} - 2 \frac{\nrm{w^2 - m}^2}{h(w)^3} \grad h(w), 
%\end{align*}
%and thus, 
%\begin{align*}
%\grad^2 \Phi(w) &=  \frac{12 w^2  - 4 m}{h(w)^2} - \frac{16 w (w^2 - m)}{h^3(w)} \grad h(w)^\top - 2 \frac{\nrm{w^2 - m}^2}{h(w)^3} \grad^2 h(w) + 6  \frac{\nrm{w^2 - m}^2}{h(w)^4} \grad h(w) \grad h(w)^\top. 
%\end{align*} 
%Thus, 
%\begin{align*}
%\nrm{\grad^2 \Phi(w)} &\leq  \underbrace{\nrm*{\frac{12 w^2  - 4 m}{h(w)^2}}}_{(a)} + \underbrace{\nrm*{\frac{16 w (w^2 - m)}{h^3(w)} \grad h(w)^\top}}_{(b)} +  2 \underbrace{\nrm*{\frac{\nrm{w^2 - m}^2}{h(w)^3} \grad^2 h(w)}}_{(c)} + 6  \underbrace{\nrm*{\frac{\nrm{w^2 - m}^2}{h(w)^4} \grad h(w) \grad h(w)^\top}}_{(d)}. 
%\end{align*}
%
%We bound the terms $(a)-(d)$ separately below: 
%\begin{enumerate}[label=\(\bullet\)]
%\item Bounding \((a)\):
%\begin{align*} 
%(a) &= \nrm*{\frac{12 w^2  - 12 m}{h(w)^2} + \frac{8m}{h(w)^2}} \\
%	  &\leq  \nrm*{\frac{12 w^2  - 12 m}{h(w)^2}} + \nrm*{\frac{8m}{h(w)^2}}  \\
%	  &\leq 12 \frac{\nrm*{w^2  - m}}{h(w)^2} + 8\frac{\nrm{m}}{h(w)^2} \\ 
%	  &\leq \frac{12}{\nrm{m}} \frac{\nrm*{w^2  - m}^2}{h(w)^2} + 20\frac{\nrm{m}}{h(w)^2} && \text{(using AM \(\geq\)  GM)} \\ 
%	  &\leq 12 \frac{\Phi(w)}{\nrm{m}} + 20\frac{\nrm{m}}{h(w)^2}. 
%\end{align*}
%
%\item Bounding \((b)\): 
%\begin{align*}
%(b) = \nrm*{\frac{16 w (w^2 - m)}{h^3(w)} \grad h(w)^\top}  &= \nrm*{\frac{16 w (w^2 - m)}{h^3(w)}} \nrm*{\grad h(w)} \\
%	  &\leq \nrm*{\frac{16 w (w^2 - m)}{h^3(w)}} \nrm*{\grad h(w)}_1 \\ 
%	  &= \nrm*{\frac{16 w (w^2 - m)}{h^3(w)}}. 
%\end{align*}
%
%We conclude by noting that: 
%\begin{align*}
%\nrm*{\frac{16 w (w^2 - m)}{h^3(w)}} &\leq 16 \nrm{w}_\infty \nrm*{\frac{w^2 - m}{h^3(w)}} \\
%&= 16 \sqrt{\nrm{w^2}_\infty} \cdot  \nrm*{\frac{w^2 - m}{h^3(w)}} \\ 
%&= 8 \prn*{ \frac{\nrm{w^2}_\infty}{h^4(w)}  + {\frac{\nrm*{w^2 - m}^2}{h^2(w)}}} && \text{(using AM \(\geq \)GM)}   \\ 
%&\leq 8 \prn*{ \frac{\nrm{w^2}_2}{h^4(w)}  + \Phi(w)}  && \text{(using the fact that \(\ls_\infty \leq \ls_2\))} \\
%&\leq 8 \Phi(w) + 8 \frac{\nrm{w^2 - m}}{h^4(w)}  + 8 \frac{\nrm{m}}{h^4(w)} \\ 
%\end{align*}
%\item Bounding \((c)\): 
%\begin{align*}
%(c) &= 2 \frac{\nrm{w^2 - m}^2}{h(w)^3} \nrm*{ \grad^2 h(w)} \\ 
%	 &\leq 4 \lambda \frac{\nrm{w^2 - m}^2}{h(w)^3} && \text{(using \pref{lem:vec_sq_hessian_norm})} \\ 
%	 &\leq 4 \lambda \frac{\Phi(w)}{h(w)} 
%\end{align*} 
%
%\item Bounding \((d)\): 
%\begin{align*}
% 6 \nrm*{\frac{\nrm{w^2 - m}^2}{h(w)^4} \grad h(w) \grad h(w)^\top} 
%\end{align*}
%\end{enumerate}
%
%\ascomment{Complete this bound} 
%\end{proof} 
%

%\begin{lemma} The potential defined in \pref{eq:vec_sq_potential} has self-bounding hessian. 
%
%\ascomment{I am getting a dependence on \(\phi(w)^3\)} 
%\end{lemma}
%\begin{proof} First note that: 
%\begin{align*}
%\grad \Phi(w) &= 4 \frac{w^3 - m w}{h(w^2)} - 2 \frac{\nrm{w^2 - m}^2}{h(w^2)^2}  \diag(w) \grad h(w^2),  
%\end{align*}
%and thus, 
%\begin{align*}
%\grad^2 \Phi(w) &=  \frac{12 w^2  - 4 m}{h(w^2)} - \frac{16 w^2 (w^2 - m)}{h^2(w^2)} \grad h(w^2) - 2 \frac{\nrm{w^2 - m}}{h(w^2)^2} \grad h(w^2) \\
%& \qquad \qquad - 4 w \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \grad^2 h(w^2) + 8  \frac{\nrm{w^2 - m}^2}{h(w^2)^3} w^2 \grad h(w^2) \grad h(w^2)^\top. 
%\end{align*}
%
%Thus, 
%\begin{align*}
%\nrm{\grad^2 \Phi(w)} &\leq  \nrm*{\frac{12 w^2  - 4 m}{h(w^2)}} + 16  \nrm*{\frac{w^2 (w^2 - m)}{h^2(w^2)} \grad h(w^2)} + 2\frac{\nrm{w^2 - m}}{h(w^2)^2}  \nrm*{ \grad h(w^2)}\\
%& \qquad \qquad + 4  \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w  \grad^2 h(w^2)} + 8 \frac{\nrm{w^2 - m}^2}{h(w^2)^3} \nrm*{   w^2 \grad h(w^2) \grad h(w^2)^\top}
%\end{align*}
%We bound each term separately below: 
%\begin{enumerate}
%\item Bound on \(\nrm*{\frac{12 w^2  - 4 m}{h(w^2)}}\)
%\begin{align*}
%\nrm*{\frac{12 w^2  - 4 m}{h(w^2)}} &\leq 12 \frac{\nrm*{w^2  - m}}{h(w^2)} + 8 \frac{\nrm*{m}}{h(w^2)}  \\
%\end{align*} 
%
%\item Boung on \(  \nrm*{\frac{w^2 (w^2 - m)}{h^2(w^2)} \grad h(w^2)} \)
%\begin{align*}
%  \nrm*{\frac{w^2 (w^2 - m)}{h^2(w^2)} \grad h(w^2)}  &\leq  \frac{\nrm*{w^2 (w^2 - m)}}{h^2(w^2)} \nrm*{\grad h(w^2)}   \\ 
%  &\leq \frac{\nrm*{w^2 (w^2 - m)}}{h^2(w^2)} && \text{(Since \(\nrm*{\grad h(w^2)} \leq 1\))}  \\
%  &\leq \frac{\nrm*{w^2} \nrm*{(w^2 - m)}}{h^2(w^2)} \\
%  &\leq \frac{1}{2} \cdot  \frac{\nrm*{w^2}^2  + \nrm*{w^2 - m}^2}{h^2(w^2)} \\
%  &\leq \frac{1}{2} \cdot  \frac{2\nrm*{m}^2  + 3\nrm*{w^2 - m}^2}{h^2(w^2)} \\
%\end{align*}
%
%\item Bound on \(\frac{\nrm{w^2 - m}}{h(w^2)^2}  \nrm*{ \grad h(w^2)}\)
%\begin{align*}
%\frac{\nrm{w^2 - m}}{h(w^2)^2}  \nrm*{ \grad h(w^2)} &\leq \frac{\nrm{w^2 - m}}{h(w^2)^2} \\
%\end{align*}
%
%\item Bound on \( \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w  \grad^2 h(w^2)}\)
%\begin{align*}
% \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w  \grad^2 h(w^2)} &\leq  \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w  \grad^2 h(w^2)} \\
% &\leq \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w}_\infty  \nrm*{\grad^2 h(w^2)}_{1, 1} \\
% &\leq \lambda \frac{\nrm{w^2 - m}^2}{h(w^2)^2} \nrm*{w}_\infty \\
% &\leq \frac{\lambda}{2} \prn[\Big]{\frac{\nrm{w^2 - m}^4}{h(w^2)^2}  + \frac{\nrm*{w}^2_\infty}{h(w^2)^2}} \\ 
% &=  \frac{\lambda}{2} \prn[\Big]{\frac{\nrm{w^2 - m}^4}{h(w^2)^2}  + \frac{\nrm*{w^2}_\infty}{h(w^2)^2}} \\
% &\leq  \frac{\lambda}{2} \prn[\Big]{\frac{\nrm{w^2 - m}^4}{h(w^2)^2}  + \frac{\nrm*{w^2}}{h(w^2)^2}} \\
%  &\leq  \frac{\lambda}{2} \prn[\Big]{\frac{\nrm{w^2 - m}^4}{h(w^2)^2}  + \frac{\nrm*{w^2 - m}}{h(w^2)^2} + \frac{\nrm{m}}{h(w^2)^2}} \\
%\end{align*}
%\item Bound on $\frac{\nrm{w^2 - m}^2}{h(w^2)^3} \nrm*{   w^2 \grad h(w^2) \grad h(w^2)^\top}$
%\begin{align*}
%\frac{\nrm{w^2 - m}^2}{h(w^2)^3} \nrm*{   w^2 \grad h(w^2) \grad h(w^2)^\top} &\leq \frac{\nrm{w^2 - m}^2}{h(w^2)^3} \nrm*{w^2} 
%\end{align*}
%\end{enumerate}
%\end{proof} 


\subsubsection{Supporting technical results}
 
\begin{lemma}
\label{lem:matrix_sqrt_h_properties}
For any point \(W\) and \(\lambda > 0\), the function \(h_\lambda\) defined in \pref{eq:matrix_sqrt_h_defn} satisfies: 
\begin{enumerate}[label=\((\alph*)\)]
\item \(h_\lambda(W)\) is in \(C_\infty\). 
\item \(h_\lambda(W) \leq \smin(M)/10\). 
\item \(\nrm{\grad h_\lambda(W)}_{F} \leq \nrm{\grad h_\lambda(W)}_{1, 1} \leq 1\). 
\item \(\grad h(W)\) is  $\lambda' = 2 \lambda \exp(\lambda \smin(M) / 10)$-Lipschitz. 
\item Provide a bound on the Lipschitz constant of \(h(W)\). 
\end{enumerate}
\end{lemma} 
\begin{proof} We derive each part separately below. 
\begin{enumerate}[label=\((\alph*)\)]
\item The proof follows trivially since both \(F(W)\) and \(h(W)\) are \(C_\infty\). 
\item By definition, we have that 
\begin{align*} 
h_{\lambda}(W) &\leq  \min \crl*{ \smin(W), \frac{\smin(M)}{10}} \leq \frac{\smin(M)}{10}. 
\end{align*}

\item Note that at any point \(W\), 
\begin{align*}
\grad h_\lambda(W) &= \frac{\bbI \odot \exp(-\lambda W)}{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}},
\end{align*} 
	
and thus  
\begin{align*}
\nrm{\grad h_\lambda(W)}_{1, 1} &= \frac{\trace{\exp(-\lambda W)}}{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}} \leq 1. 
\end{align*}
\item We prove the desired by invoking \pref{lem:ratio_property_sb} with the function \(f(W) = \bbI \odot \exp(-\lambda W)\) and the function \(g(W) = \trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}\). First note that both \(f(W)\) and \(g(W)\) are \(\lambda\)-Lipschitz. \pref{lem:ratio_property_sb} thus implies that then function \(\grad h(W) = f(W) / g(W)\) is \(L\)-Lipschitz, where 
\begin{align*} 
L &= \frac{\lambda}{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}} + \lambda  \frac{ \nrm*{\bbI \odot \exp(-\lambda W)}}{(\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}})^2} \\
&\leq \frac{2\lambda}{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}} \\
&\leq 2 \lambda \exp(\lambda \smin(M) / 10). 
\end{align*} 

% 
% Consider any point \(\bW\), and note that 
%\begin{align*}
%	\nrm{\grad h(W) - \grad h(\bW)}  &= \nrm*{\frac{\bbI \odot \exp(-\lambda W)}{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}}  - \frac{\bbI \odot \exp(-\lambda \bW)}{\trace{\exp(- \lambda \bW)} + \exp\prn*{- {\lambda \smin(M)}/{10}}}}  \\
%	% &=\nrm*{\frac{\bbI \odot \exp(-\lambda W) \prn{\trace{\exp(- \lambda \bW)} + \exp\prn*{- {\lambda \smin(M)}/{10}}} - \bbI \odot \exp(-\lambda \bW) \prn{\trace{\exp(- \lambda W)} + \exp\prn*{- {\lambda \smin(M)}/{10}}}}{\trace{\exp(- \lambda \bW)} + \exp\prn*{- {\lambda \smin(M)}/{10}} }} 
%\end{align*} 


\end{enumerate} 
\end{proof} 

%\begin{lemma} 
%\label{lem:vec_sq_hessian_norm} The matrix \(\grad^2 h(w)\) defined in \pref{eq:vec_sq2} satisfies 
%\begin{align*}
%	\nrm{\grad^2 h(w)} \leq 2 \lambda. 
%\end{align*} 
%\end{lemma} 
%\begin{proof} 
%\begin{align*} 
%[\grad^2 h(\omega)]_{i, j} =  \begin{cases} \frac{ - \lambda \sum_{k \neq j} e^{-\lambda \omega[k] - \lambda \omega[j]} }{\prn{\sum_{k=1}^d e^{- \lambda \omega[k]}}^2} & \text{for \(i = j\)} \\
%\frac{\lambda e^{-\lambda \omega[i] - \lambda \omega[j]} }{ \prn{\sum_{k=1}^d e^{- \lambda \omega[k]}}^2} 	& \text{for \(i \neq j\)}	 \numberthis \label{eq:vec_sq2}
%\end{cases}. 
%\end{align*}
%
%Note that we can write: 
%\begin{align*}
%\frac{1}{\lambda} \grad^2 h(w) &= \grad h(w) \grad h(w)^\top - \diag\prn*{\frac{e^{-\lambda w[i]}}{\prn{\sum_{k=1}^d e^{-\lambda w[k]}}}}. 
%\end{align*}
%	
%And thus, we have that: 
%\begin{align*}
%\nrm{ \grad^2 h(w) } &= \lambda \nrm{\grad h(w) \grad h(w)^\top - \diag\prn*{\frac{e^{-\lambda w[i]}}{\prn{\sum_{k=1}^d e^{-\lambda w[k]}}}} } \\
%&\leq \lambda \prn*{ \nrm*{\grad h(w)}^2 + 1}  \\
%&\leq \lambda \prn*{ \nrm*{\grad h(w)}_1^2 + 1}  \\
%&\leq 2 \lambda. 
%\end{align*} 
%\end{proof}

The following technical relationships will be useful in self bounding the gradient and the hessian of the potential function. 
\begin{lemma}
\label{lem:matrix_sqrt_support1} 
For any point \(W\), the following relations hold: 
\begin{enumerate}[label=\((\alph*)\)]
\item $$\frac{1}{h(W^2)} \leq \frac{\Phi(W)}{h(M)^2} + \frac{2}{h(M)}. $$
\item 
$$ \frac{\nrm{W}^2_2}{h(W^2)} \leq \frac{4 \nrm{M}_2}{h(M)^2} \Phi(W)  +  \frac{4 \nrm{M}_2}{h(M)}. $$ 
\end{enumerate} 


	
\end{lemma}
\begin{proof} We derive the three parts separately below: 
\begin{enumerate}[label=\((\alph*)\)] 
\item 
Using the first order Taylor expansion, there exists some matrix \(Z\) such that 
\begin{align*}
\abs{h_\lambda(W^2) - h_\lambda(M)} &= \abs{\tri{ \grad h(Z), W^2 - M}} \\ 
&\leq \nrm{\grad h(Z)}_F \nrm{W^2 - M}_F \\ 
&\leq \nrm{W^2 - M}_F. && \text{(using \pref{lem:matrix_sqrt_h_properties})}. 
\end{align*}

Plugging in the above in the potential function \(\Phi\), we note that 
\begin{align*} 
\Phi(W) &= \frac{\nrm{W^2 - M}^2}{h(W^2)} \geq \frac{\abs{h(W^2) - h(M)}^2}{h(W^2)} \geq  \frac{h(M)^2}{h(W^2)} - 2 h(M), 
\end{align*} where the first inequality above holds due to the fact that \(h_\lambda\) is \(1-\)Lipschitz (\pref{lem:matrix_sqrt_h_properties}). Rearranging the terms gives the desired relation. 

\item Note that  
\begin{align*}
\frac{\nrm{W}^2_2}{h(W^2)} = \frac{\nrm{W^2}_2}{h(W^2)} &\leq \frac{\nrm{W^2 - M}_2 + \nrm{M}_2}{h(W^2)} \\ 
&\leq \frac{\nrm{W^2 - M}_F}{h(W^2)} + \frac{\nrm{M}_2}{h(W^2)} \\ 
&\leq  \frac{\nrm{W^2 - M}^2_F}{4\nrm{M}_2 h(W^2)} + \frac{2\nrm{M}_2}{h(W^2)} \\
&\leq \frac{\Phi(W)}{4 \nrm{M}_2} + 2 \nrm{M}_2 \prn[\Big]{\frac{\Phi(W)}{h(M)^2} + \frac{2}{h(M)}} ,
\end{align*} where the first equality holds because \(W\) is symmetric. The inequality in the first line is due to Triangle inequality, the second line due to the fact that Frobenius norm is always larger than the spectral norm, and the third line due to AM-GM inequality. Finally, the last inequality follows from plugging in the definition of \(\Phi(W)\) and the relation in part-(a) of this lemma. Rearranging the terms and using \(h(M) \leq \smin(M) \leq \nrm{M}_2\), we get 
\begin{align*} 
\frac{\nrm{W}^2_2}{h(W^2)} &\leq \Phi(W) \prn[\Big]{\frac{1}{4 \nrm{M}_2} + \frac{2 \nrm{M}_2}{h(M)^2}}  + \frac{4 \nrm{M}_2}{h(M)} \leq  \frac{4 \nrm{M}_2}{h(M)^2} \Phi(W)  +  \frac{4 \nrm{M}_2}{h(M)}. 
\end{align*} 
\end{enumerate}




\end{proof} 


\subsubsection{Self-bounding property for the potential function} 
In the following, we show that the potential \(\Phi(\cdot)\) defined above has self-bounding gradients and hessian. In the following, we first show a bound on the gradient norm. 

\begin{lemma}[Gradient-norm is self-bounded]
\label{lem:gradient_sb_vec} 
For any point \(W\),  the potential function \(\Phi(\cdot)\) defined in \pref{eq:matrix_sqrt_potential_def} satisfies, 
\begin{align*}
\nrm{\grad \Phi(W)} &\leq \prn*{\frac{4 \nrm{M}_2 + 1}{h(M)^2}} \Phi(W)^2 + \prn*{\frac{10 \nrm{M}_2 + 6 \nrm{M}^2_2}{h(M)^2} }\Phi(W) + \frac{8 \nrm{M}_2}{h(M)}. 
\end{align*} \end{lemma} 
\begin{proof} At any point \(W\), 
\begin{align*}
\grad \Phi(W) &= \frac{2 (W^2 - M)W + 2 W (W^2 - M)}{h(W^2)} - \frac{2 \Phi(W)}{h(W^2)} \grad h(W^2) W.  
\end{align*} Thus, Triangle inequality implies that 
\begin{align*} 
\nrm{\grad \Phi(W)}_F &\leq \frac{2 \nrm{(W^2 - M)W}_F}{h(W^2)} +  \frac{2 \nrm{W(W^2 - M)}_F}{h(W^2)} + \frac{2 \Phi(W)}{h(W^2)} \nrm{\grad h(W^2) W}_F \\
&\overleq{\proman{1}} \frac{4 \nrm{W}_2 \nrm{W^2 - M}_F}{h(W^2)}  + \frac{2 \Phi(W)}{h(W^2)} \nrm{\grad h(W^2)}_F \nrm{W}_2 \\
&\overleq{\proman{2}} \frac{2 \nrm{W}^2_2}{h(W^2)} + \frac{2 \nrm{W^2 - M}^2_F}{h(W^2)}  + 2 \Phi(W) \frac{\nrm{W}_2}{h(W^2)}  \\
&\overleq{\proman{3}} \frac{2 \nrm{W}^2_2}{h(W^2)} + 2 \Phi(W)  +  \Phi(W) \prn[\Big]{\frac{\nrm{W}^2_2}{h(W^2)} + \frac{1}{h(W^2)}}  
\end{align*} 
where \(\proman{1}\) follows from Holder's inequality.  Inequality \(\proman{2}\) holds due to AM-GM inequality and due to the fact that \(\nrm{\grad h(W^2)}_F  \leq 1\) (\pref{lem:matrix_sqrt_h_properties}). \(\proman{3}\) again uses AM-GM inequality and the definition of \(\Phi(W)\). Plugging in the bounds from \pref{lem:matrix_sqrt_support1} in the above, we get 
\begin{align*}
\nrm{\grad \Phi(W)}_F \leq \frac{8 \nrm{M}_2}{h(M)^2} \Phi(W)  +  \frac{8 \nrm{M}_2}{h(M)} + 2 \Phi(W) + \Phi(W) \prn[\Big]{ \frac{\Phi(W)}{h(M)^2} + \frac{2}{h(M)} +  \frac{4 \nrm{M}_2}{h(M)^2} \Phi(W)  +  \frac{4 \nrm{M}_2}{h(M)}}.
\end{align*}
 



Collecting all the terms, we get that  
\begin{align*}
\nrm{\grad \Phi(W)} &\leq \prn*{\frac{4 \nrm{M}_2 + 1}{h(M)^2}} \Phi(W)^2 + \prn*{\frac{8 \nrm{M}_2 + 2 h(M)^2 + 2h(M) + 4 \nrm{M}_2 h(M)}{h(M)^2} }\Phi(W) + \frac{8 \nrm{M}_2}{h(M)}  \\
&\leq \prn*{\frac{4 \nrm{M}_2 + 1}{h(M)^2}} \Phi(W)^2 + \prn*{\frac{10 \nrm{M}_2 + 6 \nrm{M}^2_2}{h(M)^2} }\Phi(W) + \frac{8 \nrm{M}_2}{h(M)}.  
\end{align*} 
\end{proof}

Next, we show a bound on the hessian norm. 
\begin{lemma}[Hessian-norm is self-bounded] 
\label{lem:hessian_sb_vec} 
For any point \(w\),  the potential function \(\Phi(\cdot)\) defined in \pref{eq:vec_sq_potential} satisfies, 
\begin{align*}
\nrm{\grad^2 \Phi(w)} &\leq \alpha_3 \Phi(w)^3 + \alpha_2 \Phi(w)^2 + \alpha_1 \Phi(w) + \alpha_0, \end{align*} where the coefficients \(\crl{\alpha_j}_{j=1}^4\) depend on \(m\) and \(\lambda\) but not on \(w\). 
\end{lemma}
\begin{proof} For any \(W\), 
\begin{align*}
\grad \Phi(W) &= \frac{2 (W^2 - M)W}{h(W^2)} + \frac{2 W (W^2 - M)}{h(W^2)} - \frac{2 \Phi(W)}{h(W^2)} \grad h(W^2) W. 
\end{align*} 

Since both \(F(W)\) and \(h(W)\) are in \(C_\infty\), the function  \(\Phi\) is also in \(C_\infty\). Thus, at any point \(W\), \(\nrm{\grad^2 \Phi(W)}\) denotes the Lipschitz constant of the function \(\grad \Phi(W)\). In the following, we will bound  \(\nrm{\grad^2 \Phi(W)}\) by giving a bound on the Lipschitz constant \(L_\Phi\) of the function \(\grad 
\Phi(W)\). First, define the functions \(\psi_1, \psi_2\) and \(\psi_3\) as 
\begin{align*}
\psi_1(W) \ldef{} \frac{(W^2 - M)W}{h(W^2)}, \qquad  \psi_2(W) \ldef{} \frac{W (W^2 - M)}{h(W^2)} \text{~, and} \qquad \psi_3(W) \ldef{} \frac{\Phi(W)}{h(W^2)} \grad h(W^2) W 
\end{align*} with Lipschitz constants \(L_1\), \(L_2\) and \(L_3\) respectively. Clearly, we have that 
\begin{align*}
L_\Phi \leq 2 (L_1  + L_2 + L_2). 
\end{align*} 
	
In the following, we bound \(L_1\), \(L_2\) and \(L_3\). 

\begin{enumerate} 
\item \textbf{Bound on \(L_1\):} We bound this by invoking \pref{lem:ratio_property_sb} with the function \(f(W) = W^3 - MW\) and \(g(w) = h(W^2)\). Note that \(f(W)\) is \((3 \nrm{W^2} + \nrm{M})\)-Lipschitz and \(g(w)\) is \(2 \nrm*{W}\)-Lipschitz (\pref{lem:matrix_sqrt_h_properties}). Thus, 
\begin{align*}
L_1 &\leq \frac{3 \nrm{W^2} + \nrm{M}}{h(W^2)} + 2\nrm{W} \frac{ \nrm*{W^3} + \nrm{MW}}{h^2(W^2)}  \\
&\leq \frac{3 \nrm{W^2} + \nrm{M}}{h(W^2)} + 2\nrm{W^2} \frac{ \nrm*{W^2} + \nrm{M}}{h^2(W^2)}, 
\end{align*} where the equality in the last line holds because \(W\) is symmetric. 
\item  \textbf{Bound on \(L_2\):} follows identically to the bound on \(L_1\) above. 
\item \textbf{Bound on \(L_3\):} We again bound this by invoking \pref{lem:ratio_property_sb} with the function \(f(W) =  \Phi(W) \grad h(W^2)  W\) and \(g(W) = h(W^2)\). Using the bound on Lipschitz constant of \(f\) from \pref{lem:matrix_sqrt_support3} and using the fact that \(g(w)\) is \(2\nrm*{W}\)-Lipschitz in \pref{lem:ratio_property_sb}, we get that 
\begin{align*} 
L_3 &\leq  \frac{\Phi(W) + \nrm{\grad \Phi(W)} \nrm{W} + \lambda' \Phi(W) \nrm{W^2}}{h(W^2)} + 2 \nrm{W} \frac{\nrm{\Phi(W) \grad \Phi(W) W}}{h(W^2)^2} \\
&\overleq{\proman{1}}  \frac{\Phi(W) + \nrm{\grad \Phi(W)} \nrm{W} + \lambda' \Phi(W) \nrm{W^2}}{h(W^2)} + 2 \Phi(W) \nrm{W}^2 \frac{\nrm{\grad \Phi(W)}}{h(W^2)^2} \\ 
&\overleq{\proman{2}} \Phi(W) \frac{1}{h(W^2)} + \nrm{\grad \Phi(W)} \frac{ \nrm{W}}{h(W^2)} + \lambda' \Phi(W) \frac{\nrm{W^2}}{h(W^2)} + 2 \Phi(W)  \frac{\nrm{W^2}}{h(W^2)^2}, 
\end{align*}
\end{enumerate} where \(\lambda' = 2 \lambda \exp(\lambda \smin(M) / 10)\), inequality \(\proman{1}\) follows from \Holder's inequality, \(\proman{2}\)  is due to  \pref{lem:matrix_sqrt_h_properties} and by noting that \(W\) is symmetric. 

The above bounds on \(L_1, L_2\) and \(L_3\) implies that 
\begin{align*}
L_\Phi = \text{\ascomment{Complete the bound above; It leads to a cubic polynomial}}  
\end{align*}
\end{proof}

%\begin{align*}
%\sup_{u \in \ball(1)}\lim_{t \rightarrow 0} ~  \nrm*{\frac{f(w)}{g(w)} - \frac{f(w + ut)}{g(w + ut)}} \cdot \frac{1}{\nrm*{ut}}  &\leq \frac{L_f(w)}{g(w)} + L_g(w) \frac{ \nrm*{f(w)}}{g^2(w)}. 
%\end{align*}


\begin{lemma}(Bound on Lipschitz constant) 
\label{lem:matrix_sqrt_support3} 
For any point \(W\), the Lipschitz constant of the function \(f(W) \ldef{} \Phi(W) \grad h(W^2) W\) satisfies 
\begin{align*} 
\nrm{\grad f(W)} &\leq \Phi(W) + \nrm{\grad \Phi(W)} \nrm{W} + \lambda' \Phi(W) \nrm{W^2}. 
\end{align*}, 
where \(\lambda' = 2 \lambda \exp(\lambda \smin(M) / 10)\). 
\end{lemma} 
\begin{proof} An application of Chain rule and Triangle inequality implies that   
\begin{align*}
\nrm{\grad f(W)} &\leq \nrm{\grad \Phi(W) \grad h(W^2) W} +\nrm{\Phi(W) \grad^2 h(W^2) W^2}  + \nrm{\Phi(W) \grad h(W^2)} \\  
&\leq  \nrm{\grad \Phi(W)} \nrm{\grad h(W^2)} \nrm{W} + \Phi(W) \nrm{\grad^2 h(W^2)}\nrm{W^2}  + \Phi(W) \nrm{\grad h(W^2)}   \\
&\leq \nrm{\grad \Phi(W)} \nrm{W} +\Phi(W) \nrm{\grad^2 h(W^2)}\nrm{W^2}  + \Phi(W) 
\end{align*}
where the inequality in the last line is due to \pref{lem:matrix_sqrt_h_properties}. Plugging in the bound on \(\nrm{\grad \Phi(W)}\) from \pref{lem:gradient_sb_vec} and \(\nrm{\grad^2 h(W)}\) from \pref{lem:matrix_sqrt_h_properties}, we get that 
\begin{align*}
\nrm{\grad f(W)} &\leq \Phi(W) + \nrm{\grad \Phi(W)} \nrm{W} + 2 \lambda \exp(\lambda \smin(M) / 10) \Phi(W) \nrm{W^2}. 
\end{align*}
\end{proof}

%\begin{proof} For any direction \(u\), and \(t \geq 0\) and for the point \(\bw = w + ut\) note that 
%\begin{align*} 
%\nrm{f(w) - f(\bw)} &= \nrm{ \Phi(w)  \diag(w) \grad h(w^2) -  \Phi(\bw)  \diag(\bw) \grad h(\bw^2)} \\  
%&\leq  \nrm{( \Phi(\bw)  \diag(\bw) -  \Phi(w)  \diag(w))\grad h(\bw^2)} + \nrm{\Phi(w)  \diag(w)}  \nrm{\grad h(w^2) - \grad h(\bw^2)} \\
%&\leq   \nrm{\Phi(\bw)  \diag(\bw) -  \Phi(w)  \diag(w)} \nrm{\grad h(\bw^2)}_1 +  \nrm{\Phi(w)} \nrm{w}_\infty  \nrm{\grad h(w^2) - \grad h(\bw^2)} \\ 
%&\leq  \nrm{\Phi(\bw)  \diag(\bw) -  \Phi(w)  \diag(w)} + \nrm{\Phi(w)} \nrm{w}_\infty  \nrm{\grad h(w^2) - \grad h(\bw^2)},
%\end{align*} where the last inequality is due to the expression in \pref{eq:vec_sq1}. We bound the terms \((a)\) and \((b)\) separately below. We thus have that: 
%\begin{align*}
%\sup_{u \in \ball(1)} \lim_{\substack{t \rightarrow 0 \\ \bw = w + ut}} \frac{\nrm{f(w) - f(\bw)}}{\nrm{w - \bw}} &\leq \overbrace{\sup_{u \in \ball(1)}  \lim_{\substack{t \rightarrow 0 \\ \bw = w + ut}} \frac{\nrm{\Phi(\bw)  \diag(\bw) -  \Phi(w)  \diag(w)} }{\nrm{w - \bw}}}^{(a)} \\
%& \qquad \qquad + \\
%& \underbrace{\sup_{u \in \ball(1)}  \lim_{\substack{t \rightarrow 0 \\ \bw = w + ut}} \frac{ \nrm{\Phi(w)} \nrm{w}_\infty  \nrm{\grad h(w^2) - \grad h(\bw^2)}}{\nrm{w - \bw}}}_{(b)} 
%\end{align*} 
%
%\begin{enumerate}
%\item \textit{Bound on term-(a):} Since \(\Phi(w)\) and \(\diag(w)\) are continuous functions, we immediately have that 
%\begin{align*}
%(a) &\leq \Phi(w) + \nrm{\grad \Phi(w) \diag(w)} \\
%&\leq \Phi(w) + \nrm{w}_\infty \nrm{\grad \Phi(w)}  \\ 
%\end{align*}
%\item \textit{Bound on term-(b):}
%\begin{align*}
%(b) &\leq 2 \nrm{\Phi(w)} \nrm{w}_\infty \nrm{\grad^2 h(w) w} \\
%&\leq 2 \nrm{\Phi(w)} \nrm{w}_\infty \nrm{w}_\infty \nrm{\grad^2 h(w)} \\
%&\leq 4 \lambda \nrm{\Phi(w)} \nrm{w}_\infty, 
%\end{align*} where the last inequality is due to \pref{lem:vec_sq_hessian_norm}. 
%\end{enumerate}
%\end{proof}


==> files/appx_applications_phase_retreival.tex <==
\subsection{Phase Retrieval}
We consider the expected loss for the phase retrieval problem: 
\begin{align*}
F(w) = \En_{a \sim \cN(0, \bbI_d)} \brk*{\prn*{(a^\top w)^2 - (a^\top w^*)^2}^2}.  \numberthis \label{eq:phase_retrieval_objective} 
\end{align*}

The following technical lemma establishes some useful properties of \(F(w)\). 
\begin{lemma} 
\label{lem:phase_ret_F_dist_relation} 
Let \(\nrm{w^*}=1\) and let \(F(w)\) denote the function given in \pref{eq:phase_retrieval_objective}. Then, for any \(w\), 
\begin{enumerate}[label=\((\alph*)\)] 
\item \(F(w) = w^\top (\bbI - (w^*)(w^*)^\top) w + \frac{3}{4} \prn*{\nrm{w}^2 - 1}^2\). 
\item \(F(w) \geq \prn*{\nrm{w}^2 - \nrm{w^*}^2}^2\). 
\item  $F(w) \leq  4d \prn*{\dist(w, w^*)^4 + 2 \dist(w, w^*)^2},$ where the distance function is defined as \(\dist(w, w^*) = \min\crl{\nrm{w - w^*}, \nrm*{w + w^*}}\).  
\end{enumerate}

\end{lemma} 
\begin{proof} We prove each part separately below: 
\begin{enumerate}
	\item The computation is straightforward. We refer the reader to Section 2.3 of \citet{candes2015phase} for the proof.   
	\item We note that 
\begin{align*}
F(w) &= \En_{a} \brk*{\prn*{(a^\top w)^2 - (a^\top w^*)^2}^2} \\
		&= \En_{a} \brk*{ \tri*{a, w - w^*}^2 \tri*{a, w + w^*}^2} \\
		&\leq \En_{a} \brk*{ \nrm{a}^4} \nrm{w - w^*}^2 \nrm*{w + w^*}^2 \\
		&\leq 2d \cdot \nrm{w - w^*}^2 \nrm*{w + w^*}^2,  \numberthis \label{eq:phase_ret1} 
\end{align*}
where the inequality in the second line holds because \(\nrm{a}^2\) is distributed according to a Chi-square distribution with \(d\) degrees of freedom. We next bound $\nrm{w - w^*} \nrm*{w + w^*}$ by \(\dist(w, w^*)\). Note that \(\dist(w, w^*) = \min\crl{\nrm{w - w^*}, \nrm*{w + w^*}}\). We assume two cases below: 
\begin{enumerate}
\item Case1: \(\dist(w, w^*) = \nrm{w - w^*}\). Here, we have: 
\begin{align*} 
\nrm{w - w^*} \nrm*{w + w^*} &= \nrm{w - w^*} \nrm*{w - w^* + 2w^*}  \\
&\leq \nrm{w - w^*}^2 + 2\nrm{w - w^*} \nrm{w^*} \\
&= \nrm{w - w^*}^2 + 2\nrm{w - w^*}  \\
&= \dist(w, w^*)^2 + 2 \dist(w, w^*), 
\end{align*} where the first inequality above holds by Triangle inequality, the second to last line holds because \(\nrm{w^*} = 1\) and the last line follows from the fact that \(\dist(w, w^*) = \nrm{w - w^*}\). 
\item Case2: \(\dist(w, w^*) = \nrm{w + w^*}\). Here, we have: 
\begin{align*}
\nrm{w - w^*} \nrm*{w + w^*} &= \nrm{w + w^* - 2w^*} \nrm*{w + w^*}  \\
&\leq \nrm{w + w^*}^2 + 2 \nrm{w^*}  \nrm{w + w^*}\\
&= \nrm{w + w^*}^2 + 2\nrm{w + w^*}  \\
&= \dist(w, w^*)^2 + 2 \dist(w, w^*), 
\end{align*} where the first inequality above holds by Triangle inequality, the second to last line holds because \(\nrm{w^*} = 1\) and the last line follows from the fact that \(\dist(w, w^*) = \nrm{w + w^*}\). 
\end{enumerate}

The two cases above imply that: 
\begin{align*}
\nrm{w - w^*} \nrm*{w + w^*} &\leq \dist(w, w^*)^2 + 2 \dist(w, w^*) .
\end{align*} Plugging which in \pref{eq:phase_ret1} implies that: 
\begin{align*} 
F(w) &\leq 2d \prn*{\dist(w, w^*)^2 + 2 \dist(w, w^*)}^2 \\
&\leq 4d \prn*{\dist(w, w^*)^4 +2 \dist(w, w^*)^2}. 
\end{align*}
The proves the first part. For the second part, note that
\begin{align*}
F(w) &= \En_{a} \brk*{\prn*{(a^\top w)^2 - (a^\top w^*)^2}^2} \\
&\geq \prn*{ \En_{a} \brk*{ (a^\top w)^2 - (a^\top w^*)^2}}^2 \\
&= \prn*{\nrm{w}^2 - \nrm{w^*}^2}^2,  
\end{align*} where the second line follows from Jensen's inequality and the last line holds because for any vector \(u\), we have \(\En_{a \sim \cN(0, \bbI)} \brk*{(a^\top u)^2} = \nrm*{u}^2\). 
\end{enumerate}
\end{proof}

Recall that we defined 
\begin{align*} 
h(w) = \sigma \prn*{-\frac{1}{2} \log\prn[\Bigg]{\exp\prn[\Big]{- 2{\tri{w, w^*}}^2 + \frac{2}{d \log(d)}} + \exp\prn[\Big]{ - \frac{2}{\log^2(d)} + 2 (1 - \nrm{w})^2}}}, 
\end{align*} and note that 
\begin{align*}
h(w) \leq \sigma \prn*{\min\crl*{ {\tri{w, w^*}}^2 - \frac{1}{d \log(d)} ,  \frac{1}{\log^2(d)} - (1 - \nrm{w})^2 }}, 
\end{align*}
where 
\begin{align*}
\sigma(z) \ldef{} \begin{cases} 
 0 & \text{if} \quad z \leq 0 \\ 
	2z^2 & \text{if} \quad 0 \leq z \leq 1/ 2  \\
	- 2z^2 + 4z - 1 & \text{if} \quad 1/2 \leq z  \leq 1 \\ 
	1 & \text{if} \quad 1 \leq z 
\end{cases}. 
\end{align*}

Furthermore, 
\(R(w ,t) = c_1 d^{c_2} e^{- c_3 t} (1 + F(w(0))\) and thus 
\begin{align*}
\Gamma(w(0)) &= \frac{c_1 d^{c_2}}{c_3} \cdot (1 + F(w(0))
\end{align*}
\subsubsection{Rate of convergence for gradient flow} 

\begin{lemma}[Phase Retrieval gradient flow rate]
Let \(\nrm{w^*}=1\) and let \(w(0)\) be any initial point that satisfies \(\tri{w(0), w^*}^2 \geq \frac{1}{d \log(d)}\) and \((1 - \nrm{w(0)}))^2 \leq \frac{1}{\log^2(d)}\). Then, the point \(w(t)\) returned by gradient flow after time \(t\) satisfies \begin{align*} 
F(w) \leq  c_1 d^{c_2} e^{- c_3 t} (1 + F(w(0))), 
\end{align*} where \(c_1, c_2\) and \(c_3\) are universal constants independent of \(d\).
%
% initialization that satisfies  let \(F(w)\) denote the function given in \pref{eq:phase_retrieval_objective}. Then, for any \(w\) that satisfies \(\abs*{w - 1} \leq \frac{1}{\log(d)}\), we have 
%\begin{align*}
%\nrm{w} \leq \frac{1}{2} \log(d) F(w). 
%\end{align*}
\end{lemma} 
\begin{proof} We start from the convergence guarantee in \cite{chen2019gradient}. In particular, Theorem 2 there implies that whenever \({\tri{w(0), w^*}}^2 \geq \frac{1}{d \log(d)}\) and \(\frac{1}{\log^2(d)} \geq (1 - \nrm{w(0)}))^2\), we have that gradient flow satisfies the convergence guarantee: 
\begin{align*}
\dist(w(t), w^*) &\leq e^{- c(t - \log(d))}, 
\end{align*}
where we plugged in \(T_\gamma = \log(d)\) and \(\gamma = 1\) in the Theorem 2 guarantee and note that \(c\) is a universal constant. Using the above bound with \pref{lem:phase_ret_F_dist_relation}, we have that 
\begin{align*} 
F(w) &\leq 4d \prn*{\dist(w, w^*)^4 + 2 \dist(w, w^*)^2} \\
&\leq 4d^{4c + 1} e^{-4ct}  + 8 d^{2c + 1} e^{-2ct} \\ 
&\leq  4d^{4c + 1} e^{-2ct} \\
&\leq  4d^{4c + 1} e^{-2ct} (1 + F(w(0))), 
\end{align*} where the last line holds because \(F(w(0)) \geq 0\). 
\ascomment{Maybe this rate function can be improved without this trick! Directly use the monotonicity property!} 

%We next note that the initialization \(w(0)\) satisfies: 
%\begin{align*}
%1 \leq \frac{\log(d)}{\log(d/e)}^4 \nrm{w(0)}^4 \overleq{\proman{1}} 16 \nrm{w(0)}^4  \overleq{\proman{2}} 32(F(w) + 1)
%\end{align*} where \(\proman{1}\) holds for any \(d \geq 10\) and \(\proman{3}\) holds because 
%\begin{align*}
%\nrm{w}^2 &= 1 + \sqrt{\prn*{\nrm{w^2} - 1}^2} \leq 1 + \sqrt{F(w)}. 
%\end{align*}
%where the last line holds due to \pref{lem:phase_ret_F_dist_relation}.
\end{proof} 
\subsubsection{Self-bounding regularity conditions}
We first establish the self-bounding properties for \(F(w)\) (which directly extend to the self-bounding properties of \(\Gamma(w)\)).

\begin{lemma} For any \(w\), 
\begin{align*}
\max{\crl{\nrm{\grad F(w)},  \nrm{\grad^2 F(w)}}} \leq \Lambda(\Gamma(w)), 
\end{align*}
	for some non-decreasing function \(\Lambda\). Furthermore, 
 \begin{align*}
\max{\crl{\abs*{h(w) - h(w^*)}^2, \nrm{\grad h(w)},  \nrm{\grad^2 h(w)}}} \leq \pi(\Gamma(w)), 
\end{align*}
\end{lemma}
\begin{proof} First note that 
\begin{align*}
\nrm{\grad F(w)} &\leq 2 \nrm{w} + 2 \nrm{w, w^*}^2 + 2 \nrm{w} \nrm{\nrm{w}^2 - 1}^2. 
\end{align*}
and  
\begin{align*}
\nrm{\grad^2 F(w)} &= 2  + 2  \nrm{w^*}^2 + 2 \prn{\nrm{w}^2 - 1}^2 + 2 \nrm{w}^3 \prn{\nrm{w}^2 - 1}. 
\end{align*}

The self bounding properties following by noting that: 
\begin{align*}
\nrm{w} \leq \sqrt{ \nrm{w^*}^2 + \abs{\nrm{w}^2 - \nrm{w^*}^2}} \leq \sqrt{\nrm{w^*}^2 + 4 F(w)}. 
\end{align*}

The self-bounding properties on \(\nrm{\grad h(w)}\) and \(\nrm*{\grad h(w)}\) similarly follow by using the Lipschitzness of \(h\) and using the fact that 
\begin{align*}
\nrm{w} \leq \sqrt{ \nrm{w^*}^2 + \abs{\nrm{w}^2 - \nrm{w^*}^2}} \leq \sqrt{\nrm{w^*}^2 + 4 F(w)}. 
\end{align*}

\end{proof}



\begin{proof}[Proof of \pref{thm:pr_main}] The proof follows by combining \pref{lem:indicator_utility_lemma} with \pref{thm:GD_guarantee} / \pref{thm:SGD_guarantee} with the function \(R_\pr\) and \(h_\pr\) and noting that both all the properties required in \pref{lem:indicator_utility_lemma} are satisfied. 
\end{proof}
 
 
%\subsection{Alternate version}
%
%We next derive the gradient property. 
%\begin{align*} 
%h(w) = -\frac{1}{2} \log\prn[\Bigg]{\exp\prn[\Big]{- 2{\tri{w, w^*}}^2 + \frac{2}{d \log(d)}} + \exp\prn[\Big]{2\nrm{w}^2 - 2}}
%\end{align*}
%
%\begin{align*}
%\grad h(w) &= \frac{-1}{2 \kappa} \prn*{ \exp\prn[\Big]{- 2{\tri{w, w^*}}^2 + \frac{2}{d \log(d)}} \cdot -4 \tri{w, w^*} w^* + \exp\prn[\Big]{ 2 \nrm{w}^2 - 2} \cdot 4 w}  \\
%&= \prn*{ \exp\prn[\Big]{- 2{\tri{w, w^*}}^2 + \frac{2}{d \log(d)}} \cdot \tri{w, w^*} w^* + \exp\prn[\Big]{ 2 \nrm{w}^2 - 2} \cdot - w} 
%\end{align*} 
%
%Also, 
%\begin{align*} 
%- \grad F(w) = - 2 w + 2 \tri{w, w^*} w^* - 3 \prn{\nrm{w}^2 - 1} w 
%\end{align*}
%
%We have 
%\begin{align*}
%\tri*{\grad h(w), - \grad F(w)}  &\propto  \exp\prn[\Big]{- 2{\tri{w, w^*}}^2 + \frac{2}{d \log(d)}} \cdot 3 (1 - \nrm{w}^2) \tri{w, w^*}^2 + \exp\prn[\Big]{2 \nrm{w}^2 - 2} \cdot \prn*{3 \nrm{w}^4 - 2 \tri{w, w^*} - \nrm{w}^2} 
%\end{align*}
%
%
%\section{Alternate version 3}
%The dynamics is given by 
%\begin{align*}
%&\alpha_{t+1} = \alpha_t + 3 \eta \alpha_t - 3 \eta \nrm{w_t}^2 \alpha_t  \\ 
%&\beta_{t+1} = \beta_t +  \eta \beta_t - 3 \eta \nrm{w_t}^2 \beta_t 
%\end{align*}
%
%We thus have 
%
%\begin{align*}
%&\alpha^2_{t+1} = \alpha^2_t + 9 \eta^2 \alpha^2_t + 9 \eta^2 \nrm{w_t}^4 \alpha^2_t + 6 \eta \alpha_t^2 - 6 \eta \nrm{w_t}^2 \alpha_t^2 - 18 \eta^2 \nrm{w_t}^2 \alpha_t^2 \\ 
%&\beta^2_{t+1} = \beta^2_t +  \eta^2 \beta^2_t + 9 \eta^2 \nrm{w_t}^2 \beta_t^2 + 2 \eta \beta_t^2 - 6 \eta \nrm{w_t}^2 \beta_t^2 - 6 \eta^2 \nrm{w_t}^2 \beta_t^2. 
%\end{align*} 
%
%We now evaluate 
%\begin{align*} 
%\alpha_{t+1}^2 - \kappa \beta_{t+1}^2 &= \prn*{1 + 9 \eta^2 \nrm{w_t}^4 - 6 \eta \nrm{w_t}^2 + \eta^2 + 2 \eta - 18 \eta^2 \nrm{w_t}^2} (\alpha_t^2 - \kappa \beta_t^2)  - 12 \kappa\eta^2 \nrm{w_t}^2 \beta_t^2 + 8 \eta^2 \alpha_t^2 + 4 \eta \alpha_t^2 \\ 
%&\geq  \prn*{1 + \eta( 3 \nrm{w_t}^2 - 1 )^2  - 6 \eta \nrm{w_t}^2 + 2 \eta} (\alpha_t^2 - \kappa \beta_t^2)  - 12 \eta^2 \nrm{w_t}^2 \alpha_t^2 + 8 \eta^2 \alpha_t^2 + 4 \eta \alpha_t^2 \\ 
%&\geq  \prn*{1 + \eta( 3 \nrm{w_t}^2 - 1 )^2} \prn*{\alpha_t^2 - \kappa \beta_t^2}
%\end{align*}
%









==> files/appx_ub_sgd.tex <==
\subsection{Proof of \pref{thm:SGD_guarantee}} 
We first note the following high probability and in-expectation bounds on the norm of the stochastic gradient estimate. 
\begin{lemma} 
\label{lem:SGD_bound_hp}	 
Let \(\crl*{w_t}_{t \leq T}\) be the sequence of iterates generated by SGD algorithm on \(F\) using stochastic estimates based on \(\crl{z_t}_{t \leq T}\). Then, with probability at least \(1 - \delta\), for any time \(t \leq T\), 
\begin{align*}
\nrm*{\grad f(w;z)}^2 &\leq  \Lambda(F(w)) \log\prn*{T/\delta} 
\end{align*}
and for any \(w > 0\), 
\begin{align*}
\En \brk*{\nrm{\grad f(w; z)}^2} &\leq \Lambda(F(w)), 
\end{align*}
where the function $\Lambda(z) \ldef{}  2 \psi(z) + 2\chi(z)$, and the functions \(\psi\) and \(\chi\) given in \pref{ass:F_regular} and \ref{ass:gradient_noise} respectively. 
\end{lemma} \begin{proof} Note that for any \(0 \leq t \leq T\), with probability at least \(1 - \frac{\delta}{T}\), 
\begin{align*}
\nrm*{\grad f(w; z)  - \grad F(w)}^2 &\leq \chi(F(w)) \cdot \log\prn*{\frac{T}{\delta}}, 
\intertext{which implies that}
\nrm*{\grad f(w;z)}^2 &\leq 2 \nrm*{\grad F(w)}^2  + 2 \nrm*{\grad f(w; z)  - \grad F(w)}^2 \\ 
&\leq 2 \psi(F(w)) + 2 \nrm*{\grad f(w; z)  - \grad F(w)}^2 \\ 
&\leq \prn*{2 \nrm*{\grad F(w)}^2  +  2 \chi(F(w))} \cdot \log\prn*{\frac{T}{\delta}} \\  
&= \Lambda(F(w)) \log\prn*{\frac{T}{\delta}}, 
\end{align*} where the inequality in the second to last line follows from \pref{ass:gradient_noise} and the last line is from the definition of \(\Lambda\). The desired bounds follows with probability at least \(1 - \delta\) by taking a union bound w.r.t.~\(t\). 
 

For the in-expectation bound, since for any random variable \(X\), \(\En \brk*{X} = \int_{t = 0}^\infty \Pr(X \geq t) \dif t\), we have  
\begin{align*} 
\frac{\En \brk*{\nrm{\grad f(w; z) - \grad F(w)}^2}}{\chi(F(w))} &= \int_{t=0}^\infty  \Pr \prn*{\frac{\En \brk*{\nrm{\grad f(w; z) - \grad F(w)}^2}}{\chi(F(w))}  \geq t} \dif t \\ 
&\leq \int_{t=0}^\infty  e^{- t} \dif t = 1.  \numberthis \label{eq:basic_expect1}
\end{align*}
Thus, 
\begin{align*}
\En \brk*{\nrm{\grad f(w; z)}^2} &\leq 2\nrm*{\grad F(w)}^2 + 2 \En \brk*{\nrm{\grad f(w; z) - \grad F(w)}^2} \\ &\leq  2\nrm*{\grad F(w)}^2 + 2 \chi(F(w)) \\
&\leq 2 \psi(F(w)) + 2\chi(F(w)) \rdef{} \Lambda(F(w)), 
\end{align*} where the inequality in the second line above follows \pref{eq:basic_expect1} and the last line is due to \pref{ass:gradient_noise}. 
\end{proof} 

We are now ready to prove the convergence guarantee for SGD. We first state the full version of \pref{thm:SGD_guarantee} that shows all the problem dependent constants hidden in the main body, but keeps \(\kappa\) as a free variable. Then, we provide an easier to understand result in \pref{rem:SGD_proof_corollary} by setting  \(\kappa\) appropriately. Various invocations of this result are presented in \pref{sec:applications} (with the proofs in \pref{app:applications})

\begin{theorem*}[\pref{thm:SGD_guarantee} restated with problem dependent constants] 
Let \(\Phi_g\) be an admissible potential w.r.t.~$F$. Assume that \(F\) satisfies  \pref{ass:F_regular} with the bound given by the function \(\psi\), \(\Phi_g\) satisfies \pref{ass:Phi_regular} with the bound given by the function \(\rho\), and the stochastic gradient estimates \(\grad f(w; z)\) satisfy \pref{ass:gradient_noise} with the bound given by the function \(\chi\). Then, for any \(T \geq 1\) and \(\eta \leq  \frac{M - \theta(\Phi(w_0))}{20\log(20 T) \sqrt{MBT}}\), with probability at least \(0.7\), the point \(\wh w_T\) returned by SGD algorithm satisfies for any \(\kappa > 1\), 
\begin{align*} 
\bridge{F(\wh w_T)} &\leq \kappa \rho(\Phi(w_0))  \prn*{50 \eta B + \frac{10 \taylor(\Phi(w_0))}{\eta T}}, 
\end{align*} 
where the function \(\theta(z) \ldef{} \int_{y=0}^z \frac{1}{\rho(y)} \dif y\), the function \(\zeta\) is defined such that  \(\zeta^{-1}(z) = \int_{y=0}^{z} \frac{\bridge{y}}{\psi(y)} \dif y\) and the function \(\Lambda(z) \ldef{} 2 \psi(z) + 2 \chi(z)\). Furthermore, the constant  \(B = \Lambda(\zeta(\rho^{-1}(\kappa \rho(\Phi(w_0)))))\) and \(\)
\(M = \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0))))\). 
\end{theorem*} 
\begin{remark} 
\label{rem:SGD_bound} Fix any initial point \(w_0\) and let \(\bw\) be any point such that \(\Phi(\bw) > \Phi(w_0)\). Then, setting \(\kappa = \tfrac{\rho(\Phi(\bw))}{\rho(\Phi(w_0))}\) in \pref{thm:SGD_guarantee} (above) implies that for any \(T \geq 1\) and \(\eta \leq  \tfrac{\theta(\Phi(\bw)) - \theta(\Phi(w_0))}{20\log(20 T) \sqrt{\Lambda(\zeta(\Phi(\bw))) \theta(\Phi(\bw)) \cdot T}}\), 
with probability at least \(0.7\), the point \(\wh w_T\) returned by SGD algorithm satisfies for any \(\kappa > 1\), 
\begin{align*} 
\bridge{F(\wh w_T)} &\leq \rho(\Phi(\bw))  \prn*{50 \eta \Lambda(\zeta(\Phi(\bw))) + \frac{10 \taylor(\Phi(w_0))}{\eta T}}. 
\end{align*} 
\end{remark}

\begin{proof}[Proof of \pref{thm:SGD_guarantee}]
Let \(\crl*{w_t}_{t \leq T}\) be the sequence of iterates generated by SGD algorithm in the first \(T\) times steps using the random samples \(\crl*{z_t}_{t \leq T}\) sampled i.i.d.~ from an unknown distribution. Let \(\cF_t\) be the natural filtration at time \(t\) such that \(\crl{w_{j}, z_{j}}_{j \leq t}\) are \(\cF_t\)-measurable, and let \(\bar{\eta} = \frac{M - \theta(\Phi(w_0))}{20\log(20 T) \sqrt{MBT}}\). 

\vspace{2mm} 

\textbf{Part 1: Expanding  the terms.} For any \(0 \leq t \leq T\), an application of \pref{lem:g_one_sided_smooth} with \(w = w_t\) and \(u = - \eta \grad f(w_t; z_t)\) implies that   
\begin{align*} 
\taylor(\Phi(w_{t +1})) &= \taylor(\Phi( w_t - \eta \grad f(w_t; z_t))) \\
&\leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} \tri*{\grad f(w_t; z_t),  \grad \Phi(w_t)} + \frac{\eta^2}{2}  \nrm{\grad f(w_t; z_t)}^2. \numberthis \label{eq:SGD_proof_1} 
\end{align*} 

Taking expectation on both the sides with respect to \(z_t\), we get 
\begin{align*} 
\En_t \brk*{\taylor(\Phi(w_{t +1}))} &\leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} \En_t \brk*{ \tri*{\grad f(w_t; z_t),  \grad \Phi(w_t)}} + \frac{\eta^2}{2} \En_t \brk*{ \nrm{\grad f(w_t; z_t)}^2 } \\
&\leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t)) + \frac{\eta^2}{2} \En_t \brk*{ \nrm{\grad f(w_t; z_t)}^2 } \\ 
&\leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t)) + \frac{\eta^2}{2} \En_t \brk*{ \nrm{\grad f(w_t; z_t)}^2 } \\
&\leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t)) + \frac{\eta^2}{2} \Lambda(F(w_t)),  \numberthis \label{eq:SGD_proof_14}
\end{align*} where the inequality in the second line holds because \( \En \brk*{ \tri*{\grad f(w_t; z_t),  \grad \Phi(w_t)}} = \tri{\grad F(w_t), \grad \Phi(w_t)} \geq g(F(w_t))\) since \(w_t\) is independent of \(z_t\), and the last line follows from \pref{lem:SGD_bound_hp}. Taking expectation on both the sides, rearranging the terms and telescoping $t$ from  \(0\) to \(T-1\), we get that 
\begin{align*} 
\En \brk*{ \sum_{t=0}^{T-1} \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t)) }  &\leq \Phi(w_0) - \En \brk*{\Phi(w_{T})} + \frac{\eta^2}{2} \En \brk*{\sum_{t=0}^{T-1} \Lambda(F(w_t))} \\
&\leq  \Phi(w_0) + \frac{\eta^2}{2} \En \brk*{\sum_{t=0}^{T-1} \Lambda(F(w_t))}. 
\end{align*}
An application of Markov's inequality thus implies that with probability at least \(0.9\), 
\begin{align*}
\sum_{t=0}^{T-1} \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t))  &\leq 10 \En \brk*{ \sum_{t=0}^{T-1} \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t)) }  \\ 
&\leq 10 \Phi(w_0) + 5 \eta^2 \En \brk*{\sum_{t=0}^{T-1} \Lambda(F(w_t))}.  \numberthis \label{eq:SGD_proof_11}  
\end{align*}

Furthermore, another application of Markov's inequality implies that with probability at least \(0.9\), 
\begin{align*} 
 \En \brk*{\sum_{t=0}^{T-1} \Lambda(F(w_t))} \leq 10 \sum_{t=0}^{T-1} \Lambda(F(w_t)). \numberthis \label{eq:SGD_proof_12}  
\end{align*}

\ascomment{This proof part seems to be wrong! Our applications of Markov's is wrong. This needs to be fixed everywhere!}  

Taking a union bound w.r.t.~ events in  \pref{eq:SGD_proof_11}  and \pref{eq:SGD_proof_12}, we get that with probability at least \(0.8\), 
\begin{align}
\sum_{t=0}^{T-1} \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t))  - 50 \eta^2 \sum_{t=0}^{T-1} \Lambda(F(w_t)) \leq 10 \Phi(w_0). \label{eq:SGD_proof_13}   \tag{\(\mathscr{E}_1\)} 
\end{align}

Our focus in the rest of the proof will be to control the term on the left hand size above. 

\vspace{2mm} 

\textbf{Part 2: Lower bound on \(\mb{\rho(\Phi(w_t)}\)}.  We first set up additional notation and derive some supporting results. Consider the stochastic process \(\crl{Y_t}_{t \leq T}\) defined as 
\begin{align*} 
Y_t = \begin{cases} 
\taylor(\Phi(w_{t})) + \sum_{j=0}^{t-1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}}  & \text{if \(t \leq \tau\)} \\
	Y_{\tau} & \text{if \(t > \tau\)}
\end{cases}, \numberthis \label{eq:SGD_sb_process_definition} 
\end{align*}
where \(\tau\) is defined as the first time smaller than or equal to \(T\) at which 
\begin{align*} 
\tau = \inf \crl*{ t \leq T \mid \rho(\Phi(w_t)) > \kappa \rho(\Phi(w_0))}, \numberthis \label{eq:stopping_time_SGD_sb} 
\end{align*}
where \(\kappa > 1\) and will be set later. If there is no such \(\tau\) for which  \pref{eq:stopping_time_SGD_sb} holds, we set \(\tau = T\). Essentially, \(\crl{Y_t}_{t \leq T}\) is a stochastic process where \(Y_t\) depends on the random variable  \(w_t\), and is stopped as soon as \(\rho(\Phi(w_t)) > \kappa \rho(\Phi(w_0))\). To keep the current proof concise, we show in \pref{lem:Y_t_supmartingale} (below) that the process \(\crl*{Y_t}_{t \geq 0}\) is a super-martingale with respect to the filtration \(\cF_t\), and that with probability at least \(0.95\), for all \(t \leq T\), 
\begin{align}
Y_t - Y_0 \leq \sqrt{\frac{1}{2} \sum_{j=0}^{t-1} \prn*{  5 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{j}; z_j)} + 4 \eta^2 \nrm*{\grad f(w_{j}; z_j)}^2}^2 \log(20T)}. \label{eq:SGD_proof_15}   \tag{\(\mathscr{E}_2\)}
\end{align}
where  \(M = \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0)))) \) .
We additionally also note that from \pref{lem:SGD_bound_hp}, with probability at least \(0.95\), for all \(t \leq T\), 
\begin{align}
\nrm*{\grad f(w;z)}^2 &\leq  \Lambda(F(w)) \log\prn*{20T} \label{eq:SGD_proof_16}   \tag{\(\mathscr{E}_3\)}
\end{align} 

Taking a union bound over the events \(\mathscr{E}_2\) and \(\mathscr{E}_3\) above, we get that for any \(t \leq T\), 
\begin{align}
Y_t - Y_0 &\leq \sqrt{\frac{1}{2} \sum_{j=0}^{t-1} \prn*{  5 \eta \sqrt{M \cdot \Lambda(F(w_j))} + 4 \eta^2  \Lambda(F(w_j))}^2 \log^2(20T)}. \label{eq:SGD_proof_17}   \tag{\(\mathscr{E}_4\)}
\end{align}

In the following, we show that under the event \(\mathscr{E}_4\), the condition in \pref{eq:stopping_time_SGD_sb} never occurs. Suppose the contrary is true and that \pref{eq:stopping_time_SGD_sb} occurs for some \(\tau \leq T\). Then, we have that 
\begin{align*}
Y_{\tau} - Y_0 &\leq \sqrt{\frac{1}{2}  \sum_{j=0}^{\tau -1} \prn*{  5 \eta \sqrt{M \cdot \Lambda(F(w_j))} + 4 \eta^2  \Lambda(F(w_j))}\log^2(20T)}\\
&\leq \sqrt{\frac{\tau}{2} \prn*{  5 \eta \sqrt{M B} + 4 \eta^2 B}^2 \log^2(20T)} \\
&\leq 9 \eta \sqrt{M B}  \log (20T) \cdot \sqrt{\tau}  \numberthis \label{eq:SGD_proof_18}
\end{align*} where the last line holds because \(\eta \leq \bar{\eta} \leq \sqrt{M/B}\) and in the second to last line, we used the fact that 
\begin{align*}
\Lambda(F(w_j)) \overleq{\proman{1}} \Lambda(\zeta(\Phi(w_j))) \overleq{\proman{2}} \Lambda(\zeta(\rho^{-1}(\kappa \rho(\Phi(w_0))))) \rdef{} B, \numberthis \label{eq:SGD_proof_19}
\end{align*} where \(\proman{1}\) holds due to \pref{lem:jont_sb_assumption} and \(\proman{2}\) follows from the fact that \(\rho(\Phi(w_j)) \leq \kappa \rho(\Phi(w_0))\) for all \(j < \tau\). However, from the definition of \(Y_t\), we also have that 
\begin{align*}
Y_\tau - Y_0 &= \taylor(\Phi(w_\tau)) - \taylor(\Phi(w_0)) + \sum_{j=0}^{\tau -1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}} \\
&\geq \taylor(\Phi(w_\tau)) - \taylor(\Phi(w_0)) - \sum_{j=0}^{\tau -1} \frac{\eta^2 \Lambda(F(w_j))}{2} \\
&\overgeq{\proman{1}} M - \taylor(\Phi(w_0)) - \sum_{j=0}^{\tau -1} \frac{\eta^2 \Lambda(F(w_j))}{2} \\
&\overgeq{\proman{2}} M - \taylor(\Phi(w_0)) - \frac{\eta^2 \tau B}{2}  \\
% &\geq M - \taylor(\Phi(w_0)) - \frac{\eta^2 T B}{2}  \\
&\geq \frac{M - \taylor(\Phi(w_0))}{2} \numberthis \label{eq:SGD_proof_20} 
\end{align*} where in \(\proman{1}\), we used the fact that \(\Phi(w_\tau) > \rho^{-1}(\kappa \rho(\Phi(w_0))) = M\),  \(\proman{2}\) follows by noting the bound in \pref{eq:SGD_proof_19} for any \(j < \tau\). The last line follows from the fact that \(\eta \leq \bar{\eta} \leq \sqrt{(M - \theta(\Phi(w_0))/B T}\). However, note that this leads to a contradiction as both \pref{eq:SGD_proof_18} and \pref{eq:SGD_proof_20} can not be simultaneously true when when \(\eta \leq \bar{\eta} = \frac{M - \theta(\Phi(w_0))}{20\log(20 T) \sqrt{MBT}}\). Thus, we must have that for any \(t \leq T\), 
\begin{align*}
\rho(\Phi(w_t)) \leq  \kappa \rho(\Phi(w_0)) \numberthis \label{eq:SGD_proof_sb5}
\end{align*}

In the following, we condition on the fact that \pref{eq:SGD_proof_sb5} holds, and provide a convergence guarantee for SGD.  

%and is sandwitched between \(\cF_t\)-predictable processes \(\crl*{A_t}_{t \leq T}\) and \(\crl*{B_t}_{t \leq T}\) such that 
%\begin{align*} 
%\abs*{B_t - A_t} &\leq \underbrace{4 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{t}; z_t)} +  4 \eta^2 \nrm*{\grad f(w_{t}; z_t)}^2}_{\rdef{G_t}}  \numberthis \label{eq:SGD_proof_sb1} 
%%&\leq 4 \eta \sqrt{B M}  +  4 \eta^2 B, 
%\end{align*} where \(M \ldef{} \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0))))\). 
%
%We next bound the probability that \(\rho(x_t) > \kappa \rho(w_0)\) for any \(t \leq T\). Let \(t\) be the first time when \(\rho(x_t) > \kappa \rho(w_0)\), i.e. \(t = \tau\). Thus, we must have that  
%\begin{align*}
%Y_t - Y_0 &= \taylor(\Phi(w_t)) - \taylor(\Phi(w_0)) + \sum_{j=0}^{t-1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}} \\
%&\overgeq{\proman{1}} M - \taylor(\Phi(w_0)) + \sum_{j=0}^{t-1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}} \\ 
%&\overgeq{\proman{2}} M - \taylor(\Phi(w_0)) + \sum_{j=0}^{t-1} \prn*{- \frac{\eta^2 \Lambda(F(w_j))}{2}} \numberthis \label{eq:SGD_proof_sb2} 
%\end{align*} where in \(\proman{1}\), we used the fact that \(\Phi(w_t) \leq \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0)))) = M\) when \(t = \tau\). The inequality in \(\proman{2}\) follows by ignoring positive terms on the right hand side. Furthermore note that for any \(t' < \tau\), we have \(\rho(\Phi(x_{t'})) \leq \kappa \rho(\Phi(w_0))\) for any \(t' < t\), we have that \ascomment{Take a proper union bound here} 
%\begin{align*}
%\Lambda(F(w_j)) \leq \Lambda(\zeta(\Phi(w_j))) &\geq \Lambda(\zeta(\rho^{-1}(\kappa \rho(F(w_0))))) \rdef{} B, 
%\end{align*} where the first inequality holds because 
%and thus
%\begin{align*} 
%Y_t - Y_0 &> M - \taylor(\Phi(w_0))  - \frac{\eta^2 
%B t}{2} \\
%&\geq \frac{M - \taylor(\Phi(w_0))}{2},  \numberthis  \label{eq:SGD_proof_sb3}  
%\end{align*} where the last line holds since \(\eta \leq \bar{\eta} \leq \sqrt{\prn{M - \theta(\Phi(w_0))}/{B t}}\). 
%
%\begin{align*}
%Y_t - Y_0 \leq \sqrt{\frac{1}{2} \sum_{j=0}^{t-1} \prn*{  5 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{j}; z_j)} + 4 \eta^2 \nrm*{\grad f(w_{j}; z_j)}^2} \log(1/\delta)}. 
%\end{align*} 
%
%
%In the following, we show that the event in \pref{eq:SGD_proof_sb3} occurs with probability at most \(0.1/T\). An application of Azuma's inequality together with the bound in \pref{eq:SGD_proof_sb1}  implies that
%\begin{align*}
%\Pr \prn*{Y_t - Y_0 > \frac{M - \taylor(\Phi(w_0))}{2}} &\leq \exp\prn*{- \frac{(M - \taylor(\Phi(w_0)))^2}{8 t \prn{8 \eta  \sqrt{ B M} 
%}^2}} \leq \frac{0.1}{T}, \\
%\end{align*} where the last line holds since \(\eta \leq \frac{M - \taylor(\Phi(w_0))}{25  \sqrt{B M T \log(10T)}}\). Taking a union bound over \(T\) implies that with probability at least \(0.9\), \begin{align*}
% \rho(x_t) \leq \kappa \rho(w_0) \numberthis \label{eq:SGD_proof_sb5}
%\end{align*} for all \(t \leq T\). In the following, we condition on the event \(\mathscr{E}_{(4)}\) being true, and provide the convergence guarantee for SGD. 

\textbf{Part 3: Convergence guarantee.} Starting from \pref{eq:SGD_proof_13}, we have that 
\begin{align*}
10 \Phi(w_0) &\geq \sum_{t=0}^{T-1} \prn*{ \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t))  - 50 \eta^2 \Lambda(F(w_t))} \\ 
&\overgeq{\proman{1}} \sum_{t=0}^{T-1} \prn*{ \frac{\eta}{\rho(\Phi(w_t))} g(F(w_t))  - 50 \eta^2 \Lambda(\zeta(\Phi(w_t)))} \\  
&\overgeq{\proman{2}} \sum_{t=0}^{T-1} \prn*{ \frac{\eta}{\kappa \rho(\Phi(w_0))} g(F(w_t))  - 50 \eta^2 B}  
\end{align*} where \(\proman{1}\)  follows from \pref{lem:jont_sb_assumption} and because \(\Lambda\) is monotonically increasing, and \(\proman{2}\) holds because of \pref{eq:SGD_proof_sb5} which implies that \( \Lambda(\zeta(\Phi(w_t))) \leq \Lambda(\zeta(\rho^{-1}(\kappa \rho(\Phi(w_0))))) = B\) since both \(\Lambda\) and \(\zeta\) are monotonically increasing functions. Rearranging the terms and dividing both the sides by \(\eta\) implies that  
\begin{align*}
\frac{1}{T} \sum_{t=0}^T g(F(w_t)) &\leq \kappa \rho(\Phi(w_0))  \prn*{50 \eta B + \frac{10 \taylor(\Phi(w_0))}{\eta T}}. 
\end{align*} 
Accounting for the union bounds for events \(\mathscr{E}_1\), \(\mathscr{E}_2\) , \(\mathscr{E}_3\)  and \(\mathscr{E}_4\), we get that the above bound holds with probability at least \(0.7\). 
\end{proof}

%\ascomment{Others:} 
% the second line above follows from \pref{lem:jont_sb_assumption} which implies that 
%\begin{align*}
%\nrm*{\grad f(w_t; z)}^2 &\leq  \chi(F(w_t)) \leq \chi(\zeta(\Phi(w_t))) \leq \chi(\zeta(\rho^{-1}(\kappa \rho(\Phi(w_t)))))  \rdef{} B,
%\end{align*} 
%where we used \pref{ass:gradient_noise}, \pref{lem:jont_sb_assumption}  and the definition in \pref{eq:SGD_sb_process_definition}  (with the condition in \pref{eq:stopping_time_SGD_sb}). Thus, for any \(\eta \leq \frac{M - \taylor(\Phi(w_0))}{25  \sqrt{B M T \log(10T)}} \leq \sqrt{M/B}\) we have 
%\begin{align*}
%\abs*{B_t - A_t} &\leq 8 \eta \sqrt{MB}.  \numberthis \label{eq:SGD_proof_sb2} 
%\end{align*}

The following technical result is used in the proof of \pref{thm:SGD_guarantee}. 
\begin{lemma}
\label{lem:Y_t_supmartingale} 
Suppose the premise of \pref{thm:SGD_guarantee} holds, and let \(\crl*{w_t}_{t \leq T}\) be the sequence of iterates generated by SGD algorithm on \(F\) using stochastic estimates based on \(\crl{z_t}_{t \leq T}\). Let the process \(\crl{Y_t}_{t \geq 0}\) be  defined as 
\begin{align*} 
Y_t = \begin{cases} 
\taylor(\Phi(w_{t})) + \sum_{j=0}^{t-1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}}  & \text{if \(t \leq \tau\)}\\
	Y_{\tau} & \text{if \(t > \tau\)}
\end{cases}, \numberthis \label{eq:SGD_sb_process_definition} 
\end{align*}
where \(\tau = \min \crl{T,  \inf \crl*{ t \mid \rho(\Phi(w_t)) > \kappa \rho(\Phi(w_0))}}\) and $\Lambda(z) =  2 \psi(F(w)) + 2\chi(F(w))$ where the function \(\psi\) and \(\chi\) given in \pref{ass:F_regular} and \ref{ass:gradient_noise} respectively. Then, \(\crl{Y_t}_{t \geq 0}\) is a super-martingale. Furthermore, with probability at-least \(0.95\), for all \(t \leq T\),  
\begin{align*}
Y_t - Y_0 \leq \sqrt{\frac{1}{2} \sum_{j=0}^{t-1} \prn*{  5 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{j}; z_j)} + 4 \eta^2 \nrm*{\grad f(w_{j}; z_j)}^2} \log(20T)}, 
\end{align*}
where \(M = \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0))) ) \). 
% and for any \(t \geq 0\), there exists \(\cF_t\)-predictable random variables   \(A_t\) and \(B_t\) such that 
%\begin{align*} 
%&A_t \leq Y_{t+1} - Y_t \leq B_t, 
%\intertext{and}
%&\abs*{B_t  - A_t} \leq 4 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{t}; z_t)} +  4 \eta^2 \nrm*{\grad f(w_{t}; z_t)}^2,
%\end{align*}  where \(G \ldef{} \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0))) )\).  
\end{lemma} 
\begin{proof} Let \(\cF_t\) be the natural filtration at time \(t\) such that \(\crl{w_{j}, z_{j}}_{j \leq t}\) are \(\cF_t\)-measurable.
For any \(t \geq 0\), repeating the steps till \pref{eq:SGD_proof_14} in the proof of \pref{thm:SGD_guarantee} above we get that 
\begin{align*} 
\En_t \brk*{\taylor(\Phi(w_{t +1}))} & \leq \taylor(\Phi(w_t)) - \frac{\eta}{\rho(\Phi(w_t))} \bridge{F(w_t)} + \frac{\eta^2 \Lambda(F(w_t))}{2},   \numberthis \label{eq:SGD_martingale1} 
\end{align*}
where \(\En_t\) denotes expectation w.r.t.~the random variable \(z_t\), and conditioning on \(\cF_{t-1}\). 
We first show that the process \(\crl{Y_t}_{t \geq 0}\) is a super-martingale. Note that for any time \(t \leq \tau\), 
\begin{align*} 
\En_t \brk*{Y_{t + 1}} &= \En_t \brk*{ \taylor(\Phi(w_{t +1}))} + \sum_{j=0}^{t} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}}  \\ 
&\leq \taylor(\Phi(w_t)) + \sum_{j=0}^{t-1} \prn*{\frac{\eta}{\rho(\Phi(w_j))} \bridge{F(w_j)} - \frac{\eta^2 \Lambda(F(w_j))}{2}} = Y_t, 
\end{align*}  
where the inequality in the second line above follows from \pref{eq:SGD_martingale1}. When \(t > \tau\), by definition we have that \(\En_t \brk*{Y_{t + 1}} = Y_t\). Hence, the process \(\crl{Y_t}_{t \geq 0}\) is a super-martingale. 

\paragraph{Bound on the difference sequence.} There are two cases, either (a) \(t > \tau\), or (b) \(t \leq \tau\). In the first case, \(\abs*{Y_{t + 1} - Y_t} = 0\). In the following, we  provide a bound on the difference sequence for \(t \leq \tau\). First note that 
\begin{align*}
Y_{t+1} - Y_t &= \taylor(\Phi(w_{t + 1})) - \taylor(\Phi(w_{t})) + \underbrace{\frac{\eta}{\rho(\Phi(w_t))} \bridge{F(w_t)} - \frac{\eta^2 \Lambda(F(w_t))}{2}}_{ \ldef{} C_t}. \numberthis \label{eq:SGD_martingale2} 
\end{align*} 

Note that the term \(C_t\) is \(\cF_t\)-predictable. Thus, we just need to find \(\cF_{t}\)-measurable processes \(A'_t\) and \(B'_t\) such that 
\begin{align*}
A'_t \leq \taylor(\Phi(w_{t + 1})) - \taylor(\Phi(w_{t})) \leq B'_t. 
\end{align*} Recall that an application of \pref{lem:g_one_sided_smooth} with \(w = w_t\) and \(u = - \eta \grad f(w_t; z_t)\) implies that 
\begin{align*}
\taylor(\Phi(w_{t + 1})) - \taylor(\Phi(w_{t})) &\leq - \frac{\eta}{\rho(\Phi(w_t))} \tri*{\grad f(w_t; z_t),  \grad \Phi(w_t)} + \frac{\eta^2}{2}  \nrm{\grad f(w_t; z_t)}^2\\
&\overleq{\proman{1}}  \frac{\eta}{\rho(\Phi(w_t))} \nrm*{\grad f(w_t; z_t)} \nrm*{\grad \Phi(w_t)} + \frac{\eta^2}{2}  \nrm{\grad f(w_t; z_t)}^2  \\ 
&\overleq{\proman{2}} \underbrace{\eta \sqrt{2 \taylor(\Phi(w_t))} \nrm*{\grad f(w_t; z_t)} + \frac{\eta^2}{2}  \nrm{\grad f(w_t; z_t)}^2}_{\rdef{} B'_t}\numberthis \label{eq:SGD_martingale3}, 
\end{align*} where \(\proman{1}\) above follows from Cauchy-Schwarz inequality, and \(\proman{2}\) holds due to \pref{lem:g_one_sided_smooth}. Note that  \(B'_t\) defined to be the terms on the RHS above is \(\cF_t\)-measurable. 

We next consider the lower bound on \(\taylor(\Phi(w_{t + 1})) - \taylor(\Phi(w_{t}))\). Plugging in \(w = w_{t+1}\) and  \(u = \eta \grad f(w_t; z_t)\) in \pref{lem:g_one_sided_smooth}, we get that 
\begin{align*}
\taylor(\Phi(w_t)) &= \taylor(\Phi(w_{t+1} + \eta \grad f(w_t; z_t))) \\ &\leq \taylor(\Phi(w_{t+1})) + \frac{\eta}{\rho(\phi(w_{t+1}))} \tri*{\grad \Phi(w_{t+1}), \grad f(w_{t}; z_t)} + \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2,
\intertext{rearranging the terms gives us} 
 \taylor(\Phi(w_{t+1}))  - \taylor(\Phi(w_{t})) &\geq - \frac{\eta}{\rho(\phi(w_{t+1}))} \tri*{\grad \Phi(w_{t+1}), \grad f(w_{t}; z_t)} -  \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2  \\ 
 &\overgeq{\proman{1}} - \frac{\eta}{\rho(\phi(w_{t+1}))} \nrm*{\grad \Phi(w_{t+1})} \nrm*{\grad f(w_{t}; z_t)} -  \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2 \\ 
 &\overgeq{\proman{2}} - \eta \sqrt{2 \taylor(\Phi(w_{t+1}))} \cdot \nrm*{\grad f(w_{t}; z_t)}  -  \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2 \\ 
  &= - \eta \sqrt{2 \taylor(\Phi(w_{t+1}) - \taylor(\Phi(w_t)) + \taylor(\Phi(w_t)))} \cdot \nrm*{\grad f(w_{t}; z_t)}  -  \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2 \\ 
  &\overgeq{\proman{3}} - \eta \sqrt{2 (\taylor(\Phi(w_{t+1}) - \taylor(\Phi(w_t))))} \cdot \nrm*{\grad f(w_{t}; z_t)}  - \eta \sqrt{2 \taylor(\Phi(w_t)))} \cdot \nrm*{\grad f(w_{t}; z_t)}  \\
  & \qquad \qquad \qquad \qquad \qquad -  \frac{\eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2 \\ 
    &\overgeq{\proman{4}} - \frac{\abs*{\taylor(\Phi(w_{t+1}) - \taylor(\Phi(w_t))}}{2} - \eta \sqrt{2 \taylor(\Phi(w_t)))} \cdot \nrm*{\grad f(w_{t}; z_t)} -  \frac{3 \eta^2}{2} \nrm*{\grad f(w_{t}; z_t)}^2 
   \end{align*} where \(\proman{1}\) follows from Cauchy-Schwarz inequality, and \(\proman{2}\) holds due to \pref{lem:g_one_sided_smooth}. Inequality \(\proman{3}\) follows from subadditivity of sq-root. Finally, \(\proman{4}\) follows from an application of AM-GM inequality. Rearranging the terms, we get 
\begin{align*} 
 \taylor(\Phi(w_{t+1}))  - \taylor(\Phi(w_{t})) &\geq \underbrace{- 2 \eta \sqrt{2 \taylor(\Phi(w_t)))} \cdot \nrm*{\grad f(w_{t}; z_t)} - 3 \eta^2 \nrm*{\grad f(w_{t}; z_t)}^2}_{\rdef{} A'_t}.  \numberthis \label{eq:SGD_martingale4}      
\end{align*}   
Note that  \(A'_t\), defined to be the terms on the RHS above, is \(\cF_t\)-measurable. 

The bounds in \pref{eq:SGD_martingale3} and \pref{eq:SGD_martingale4} imply that the processes \(\crl{A'_t}_{t \geq 0}\) and \(\crl{B'_t}_{t \geq 0}\) are \(\cF_t\)-measurable and satisfy 
\begin{align*} 
A'_t  \leq	 \taylor(\Phi(w_{t+1}))  - \taylor(\Phi(w_{t})) \leq B'_t 
\end{align*} for any \(t \geq 0\). Plugging this in \pref{eq:SGD_martingale2}, we get 
\begin{align*} 
A_t \ldef{} A'_t + C_t \leq Y_{t+1} - Y_{t} \leq B'_t + C_t \rdef{} B_t. 
\end{align*}

Clearly both \(A_t\) and \(B_t\) are \(\cF_t\)-measurable and satisfy 
\begin{align*}
\abs*{B_t  - A_t} &\leq 5 \eta \sqrt{\taylor(\Phi(w_t))} \cdot \nrm*{\grad f(w_{t}; z_t)} + 4 \eta^2 \nrm*{\grad f(w_{t}; z_t)}^2 \\ 
&\leq 5 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{t}; z_t)} + 4 \eta^2 \nrm*{\grad f(w_{t}; z_t)}^2,
\end{align*}  where the last line follow from the fact that \(t \leq \tau\) and thus \(\Phi(w_t) \leq \rho^{-1}(\kappa \rho(\Phi(w_0)))\) which implies that  \(\taylor(\Phi(w_t)) \leq \taylor(\rho^{-1}(\kappa \rho(\Phi(w_0))) ) \rdef{} M\) since \(\theta\) is a monotonically increasing function. 

\textbf{High probability bound.} An application of Azuma's inequality (\pref{lem:Azuma2}) implies that for any \(t \geq 0\), with probability at least \(1 - 1/20T\), 
\begin{align*}
Y_t - Y_0 \leq \sqrt{\frac{1}{2} \sum_{j=0}^{t-1} \prn*{  5 \eta \sqrt{M} \cdot \nrm*{\grad f(w_{j}; z_j)} + 4 \eta^2 \nrm*{\grad f(w_{j}; z_j)}^2}^2 \log(20T)}. 
\end{align*}
The desired statement follows by taking a union bound in the above for \(t\) from \(0\) to \(T-1\). 
\end{proof} 

